POSTURE: Pose Guided Unsupervised Domain Adaptation for Human Body Part Segmentation

Existing algorithms for human body part segmentation have shown promising results on challenging datasets, primarily relying on end-to-end supervision. However, these algorithms exhibit severe performance drops in the face of domain shifts, leading to inaccurate segmentation masks. To tackle this issue, we introduce POSTURE: \underline{Po}se Guided Un\underline{s}upervised Domain Adap\underline{t}ation for H\underline{u}man Body Pa\underline{r}t S\underline{e}gmentation - an innovative pseudo-labelling approach designed to improve segmentation performance on the unlabeled target data. Distinct from conventional domain adaptive methods for general semantic segmentation, POSTURE stands out by considering the underlying structure of the human body and uses anatomical guidance from pose keypoints to drive the adaptation process. This strong inductive prior translates to impressive performance improvements, averaging 8\% over existing state-of-the-art domain adaptive semantic segmentation methods across three benchmark datasets. Furthermore, the inherent flexibility of our proposed approach facilitates seamless extension to source-free settings (SF-POSTURE), effectively mitigating potential privacy and computational concerns, with negligible drop in performance.

==> sections/3_method.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/PIPS-method.drawio.pdf}
    \caption{ \textbf{Overview of Proposed Framework.} Our proposed algorithm \PIPS~ uses confident pseudo-labels from $\mathcal{F_{T}}$ to refine the predictions of the same on unlabeled data $\mathcal{T}$. Further, \PIPS~ leverages anatomical context of the human body through pose estimates (obtained from $\mathcal{P}$) aligned with body part segmentation masks by $\mathcal{G}$. Note that \PIPS~ can be extended to source-free settings, where $\{ x_{s}, y_{s} \}$ are absent (elaborated in Section~\ref{method-SFPIPS}). Even in the absence of source-data, the anatomical context obtained from $\mathcal{G} \circ \mathcal{P}$ acts as a strong regularizer, mitigating catastrophic forgetting and compensating for domain shifts.}
    \label{fig:method}
    \vskip -4mm
\end{figure*}

\section{Method}
\label{sec:method}

In this section, we provide a detailed description of our proposed algorithm (\PIPS) for human body part segmentation under distribution shifts. Our primary aim is to learn a human parsing model $\mathcal{F}$, which takes an RGB image $x \in$ $\mathbb{R}^{H \times W \times 3}$ as input, and predicts the segmentation mask $y = \mathcal{F}(x)$, where $y \in$ $\mathbb{R}^{H \times W \times K}$ for each of the $K$ classes. Here, $H$ and $W$ refer to the spatial dimensions of the image and the resulting segmentation output. 

We assume access to a source dataset $\mathcal{S} = \{x_{i}, y_{i}, p_{i} \}_{i=1}^{M}$, where $x_{i}$ is an RGB image, $y_{i}$ and $p_{i}$ are the corresponding segmentation masks and pose keypoints, respectively. The pose keypoints provide additional anatomical information about the human in a given image. Note that unlike the segmentation masks, the keypoints are \textit{sparse} annotations. Additionally, we are provided with an unlabeled target dataset $\mathcal{T}$, which contains images $ \{ x_{i} \}_{i=1}^{N}$ but lacks both body part segmentation masks and pose keypoint annotations. 
%\dripta{H,W not defined}
%\dripta{usage of pose keypoints not explained}

We seek to adapt a model that has been trained on the source dataset, denoted as $\mathcal{F_{\mathcal{S}}}$, to obtain improved performance on the target dataset $\mathcal{T}$, assuming the availability of source data. This adaptation process is driven by the anatomical information provided by the pose keypoints and is designed to yield superior results compared to directly applying $\mathcal{F_{\mathcal{S}}}$ on $\mathcal{T}$. Note that pose keypoints on $\mathcal{T}$ are \textit{not} available. This requires estimation of pose keypoints on $\mathcal{T}$ using a pre-trained pose estimation model $\mathcal{P}$ (Section~\ref{method-UDA-Pose}). We denote the model under adaptation for $\mathcal{T}$ as $\mathcal{F_{\mathcal{T}}}$. 

We also extend our algorithm (\PIPS) to the source-free setting \cite{liang2020we} and denote this algorithm as \PIPSSF~ (Section~\ref{method-SFPIPS}). Here, we assume that only $\mathcal{F_{S}}$ is available and do not assume the availability the source dataset $\mathcal{S}$ for our extended algorithm \PIPSSF. \\

\noindent {\bf Overview:} We propose to use an anatomy guided pseudo-labelling technique to obtain improved human body part segmentation masks on $\mathcal{T}$. We note that, using the model $\mathcal{F_{\mathcal{S}}}$ directly on $\mathcal{T}$ results in notably inaccurate segmentation masks, as qualitatively illustrated in Figure~\ref{fig:teaser_qual}. Employing these inaccurate masks as pseudo-labels for adaptation would introduce error accumulation, ultimately leading to subpar performance on $\mathcal{T}$. Consequently, we introduce \PIPS, an enhanced pseudo-labeling technique that consists of two highly effective methods to circumvent this error accumulation issue. 
\begin{itemize} 

    \item In order to exploit the anatomical information of the human body, we propose to fuse information from the estimated pose-keypoints on $\mathcal{T}$ (see Section~\ref{method-UDA-Pose}). This allows $\mathcal{F_{\mathcal{T}}}$ to understand the human body parts better and eliminate inconsistencies caused by self-learning from confident yet incorrect pseudo-labels (see Section ~\ref{method-pose2seg}). 

    \item Further, we propose to use the human pose context for reliable pseudo-label selection, thereby disallowing $\mathcal{F_{\mathcal{T}}}$ to overfit to incorrect but confident pseudo-labels (see Section ~\ref{method-RPL}).

\end{itemize}

An overview of our method is presented in Figure~\ref{fig:method}.
%\dripta{where is the anatomical information coming from? where do you get the pose from on target?}


\begin{comment}
\subsection{Image level alignment using Style Transfer}
\label{method-style}

Style-Transfer methods have been extensively used in problems involving unsupervised domain adaption \cite{atapour2018real, rodriguez2019domain, luo2020adversarial} in order to reduce the domain gap between the source and target images. The core idea is to train a model using the content from source images while adapting to the style of target images enhances the model's ability to generalize effectively to the target distribution and has been shown to be effective in prior works like \cite{kim2020learning, yang2020fda}. 

In this work, we employ AdaIN \cite{huang2017arbitrary} for obtaining style-transfer mappings between source and target distributions and vice-versa. The style transfer network $T$ takes in style images $s$ and content images $c$ in order to learn a combination that outputs the content of the latter in the style of the former. 
Mathematically, \begin{equation}
    T(c,s) = g(AdaIN(f(c), f(s)))
\end{equation} where

Here, $g$ is a randomly initialized decoder network and $f$ is a pre-trained feature extractor such as VGG-16 \cite{simonyan2014very}. $T$ is trained using a linear combination of content loss and style loss\cite{li2017demystifying}.
 
With a pre-trained style-transfer network $T$, we project the images from $\mathcal{S}$ to the style of $\mathcal{T}$ (denoted as $x_{s \shortrightarrow t}$) and minimize the loss described by Equation~\ref{eqn:sup}, 
\begin{equation}
    \mathcal{L}_{S} = \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{s \shortrightarrow t}), y) \ .
    \label{eqn:sup}
\end{equation}
Here, $\mathcal{L}_{ce}$ denotes the per-pixel cross-entropy loss.
\end{comment}

\subsection{Pre-training source model}
We initialize the weights of $\mathcal{F}_{T}$ by the weights of a model that is trained on the labelled source domain in supervised fashion, referred to as the source model. This source model ($\mathcal{F}_{S}$) is trained by minimizing the loss described by Equation~\ref{eqn:sup}. 
\begin{equation}
    \mathcal{L}_{S} = \mathcal{L}_{ce}(\mathcal{F_{S}}(x_{s}), y) \ .
    \label{eqn:sup}
\end{equation}
Here, $\mathcal{L}_{ce}$ denotes the per-pixel cross-entropy loss.


\subsection{Self-learning from pseudo-labels}
\label{method-SL-PL}
Self-learning from pseudo-labels \cite{choi2019pseudo, wang2020unsupervised, zhang2021prototypical} offers a simple yet powerful solution in semi/self-supervised learning problems. The fundamental idea here is to utilize only highly confident pseudo-labels for learning as discussed in \cite{guillory2021predicting}. Pseudo-labels on $\mathcal{T}$, denoted by $\hat{y}_{pl}$ can be obtained by \begin{equation}
    \hat{y}_{pl}(\tau) = \argmax \mathbbm{1} [ \mathcal{F_{\mathcal{T}}}(x_{t}) \geq \tau ] \; \mathcal{F_{\mathcal{T}}}(x_{t}) \ ,
    \label{eqn:SL-PL}
\end{equation}  where $\tau$ is the confidence threshold and $\mathbbm{1}[.]$ is an indicator function. Note that the quality of the pseudo-labels is a function of the confidence threshold $\tau$.

These pseudo-labels are incorporated in the adaptation process by minimizing the loss $\mathcal{L}_{pl}$ defined by Equation~\ref{eqn:tgt-PL}, 

\begin{equation}
    \mathcal{L}_{pl}(\tau) = \mathcal{L}_{ce}(\mathcal{F_{\mathcal{T}}}(x_{t}), \hat{y}_{pl}(\tau)) \ .
    \label{eqn:tgt-PL}
\end{equation}
    
However, we find that relying solely on these pseudo-labels for the adaptation process leads to sub-optimal performance, as it fails to consider any anatomical information related to the human body. Furthermore, the inclusion of highly confident but incorrect pseudo-labels can have a detrimental impact on the overall adaptation process. 


\subsection{Anatomy guided self-training}
\label{method-posecontext}

\subsubsection{Mapping pose keypoints to segmentation space}
\label{method-pose2seg}
In order to use the anatomical information from pose-keypoints for adapting our model $\mathcal{F_{T}}$ to our target dataset $\mathcal{T}$, we propose to learn a novel mapping that transforms the sparse pose keypoints to dense body part segmentation masks. We denote this mapping as $\mathcal{G} : \mathbb{R}^{P \times 2} \shortrightarrow \mathbb{R}^{H \times W \times K}$, where $P$ is the number of pose keypoints and $K$ is the number of classes in the segmentation maps, such as head, left/right leg, etc. 

The mapping $\mathcal{G}$ is learnt in a supervised fashion using our source dataset $\mathcal{S} = \{x_{i}, y_{i}, p_{i} \}_{i=1}^{M}$ by minimizing the loss in Equation~\ref{eqn:L-G}, 
\begin{equation}
        \mathcal{L_{G}} = \mathcal{L}_{ce}(\mathcal{G}(p_{j}), y_{j})  \ .
    \label{eqn:L-G}
\end{equation}
It is important to note that the learning of $\mathcal{G}$ does not use any RGB images, thus making it domain agnostic and hence, seamlessly applicable across different domains. Figure~\ref{fig:pose2seg} provides an overview for the learning algorithm of $\mathcal{G}$.

%\amit{Is this the best place to introduce the SF approach? Wouldn't it be better to do the next section first, and then have a new section on the source-free approach? I think that will help with the flow of the paper in the reviewers' minds.}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{images/PIPS-learning_G.drawio.pdf}
    \caption{ \textbf{Learning algorithm for $\mathcal{G}$}. The model $\mathcal{G}$ is designed by predict segmentation maps $\hat{s} \in \mathbb{R}^{H \times W \times K}$ given pose keypoints $p \in \mathbb{R}^{P \times 2}$. $\mathcal{G}$ is trained using the cross-entropy loss with ground-truth segmentation maps $s \in \mathbb{R}^{H \times W \times K}$.}
    \label{fig:pose2seg}
    \vskip -4mm
\end{figure}

Using the learned mapping $\mathcal{G}$ we can extract anatomically plausible pseudo-labels on the target dataset $\mathcal{T}$, however, this requires access to pose keypoint annotations on $\mathcal{T}$. Since we do not have access to any annotations on $\mathcal{T}$, we propose to estimate the same using a pre-trained pose estimation model which has been adapted on $\mathcal{T}$ (see Section ~\ref{method-UDA-Pose} for details).

%The learned mapping $\mathcal{G}$ is now used to extract pseudo-labels for target images $x_{t}$ via a pretrained human pose estimation model $\mathcal{P}$ (see Section ~\ref{method-UDA-Pose}). 

Mathematically, pseudo-labels $\hat{y}_{p2s}$ are obtained by \begin{equation}
    \hat{y}_{p2s} = \mathcal{G} \circ \mathcal{P} (x_{t}) \ ,
    \label{eqn:p2s}
\end{equation} and are used in the adaptation process by minimizing the loss function described in Equation~\ref{eqn:L-P2S}, 

%\dripta{describe pose more: why do you use it? how do you obtain it (in brief) Maybe add a sentence: Let us assume that we have access to a pose estimation model.... We describe the details of how to obtain this model in Sec x.}

\begin{equation}
    \mathcal{L}_{p2s} = \mathcal{L}_{ce}(\mathcal{F_{\mathcal{T}}}(x_{t}), \hat{y}_{p2s})
    \label{eqn:L-P2S} \ .
\end{equation} 

We observe that by incorporating the loss function described in Equation~\ref{eqn:L-P2S} with the losses in Equations~\ref{eqn:sup} and~\ref{eqn:tgt-PL} helps $\mathcal{F_{T}}$ achieve significant gains over the base source model. However, simply incorporating the pose information as a regularizer is not sufficient as $\mathcal{F_{T}}$ might still overfit to highly-confident incorrect pseudo-labels, driving $\mathcal{F_{T}}$ to perform sub-optimally. Therefore, we suggest leveraging the anatomical context derived from Equation~\ref{eqn:p2s} to enhance the refinement of pseudo-labels $\hat{y}_{pl}$ and thereby drive additional performance improvements.

\subsubsection{Pose-guided reliable pseudo-label selection}
\label{method-RPL}
In order to make our method more robust to incorrect pseudo-labels, we wish to employ an approach that helps $\mathcal{F_{T}}$ avoid learning from highly-confident incorrect pseudo-labels. We argue that the quality of pseudo-labels obtained using Equation~\ref{eqn:SL-PL} on a given batch of images from $\mathcal{T}$ is not homogeneous. In other words, for a batch of target images, a single threshold parameter $\tau$ may not be an optimal choice. Taking inspiration from Karim {\it et. al.} \cite{karim2023c}, we argue that any batch of target images consists of reliable and unreliable samples. In other words, predictions for some samples are relatively more accurate as compared against other samples from the same batch. Thus, we propose to split a given batch of target images (denoted by $x_{t}^{\mathbf{B}}$, containing $\mathbf{B}$ images) into reliable and unreliable splits containing $\mathbf{B}^{r}$ and $\mathbf{B}^{u}$ images respectively.

These splits are obtained by comparing the mIoU \cite{rezatofighi2019generalized} of the predictions $\mathcal{F_{T}}(x_{t})$ with $\hat{y}_{p2s}$. Essentially, for the $j^{th}$ image in a batch of target images, we obtain a score $h^{j}$ defined by Equation~\ref{miou-com},
\begin{equation}
    h^{j} = mIoU(\mathcal{\argmax(F_{T}}(x^{j}_{t})), \hat{y}^{j}_{p2s}) \ .
    \label{miou-com}
\end{equation}

This score $h^{j}$ is then used to decompose a batch of $\mathbf{B}$ images into reliable and unreliable splits as follows, 
\begin{equation}
        x_{t}^{\mathbf{B}}= 
\begin{dcases}
     x_{t}^{r}, & \text{$h_{j}$} \geq \gamma\\
     x_{t}^{u}, & \text{otherwise}
\end{dcases} \ ,
\label{eqn:split}
\end{equation}
where $\gamma$ is the threshold defining the boundary between reliable and unreliable samples. 

This is followed by extracting the confident pseudo-labels using Equation~\ref{eqn:SL-PL} with confidence thresholds $\alpha$ and $\beta$ with $\beta \geq \alpha$, for reliable and unreliable splits respectively. These pseudo-labels are now incorporated into the framework using the loss function defined below,
\begin{equation}
    \begin{split}
        \mathcal{L}_{Rpl} & = \lambda \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{t}^{r}), \hat{y}_{pl}(\alpha)) \\
        & + (1 - \lambda) \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{t}^{u}),  \hat{y}_{pl}(\beta)) \ .
    \label{eqn:loss-RPL}
    \end{split}
\end{equation}
%
Here, $\lambda$ is set to $\frac{|\mathbf{B^{r}}|}{|\mathbf{B}|}$. We experimentally demonstrate that this strategy of pseudo-label selection during adaptation contributes significantly to the overall performance gains of \PIPS~. %and \PIPSSF. %\amit{Again, I think it will be clearer if we just explain \PIPS~ first, and then go to the source-free version.}
%\calvin{Instead of moving to the source free setting and then outlining  the  objective function maybe introduce the standard objective $\shortrightarrow$ source free extention $\shortrightarrow$ source free objective}
\begin{comment}
\begin{figure}[!htb]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/Teaser final sf_posture.png}
    \caption{{\bf Overview of \PIPSSF~.} We extend our problem definition to look into source-free UDA for human body part segmentation, thereby addressing privacy and storage bottlenecks associated with using source data for adaptation as in \PIPS~.}
    \label{fig:teaser_sfposture}
\end{figure}
\end{comment}
    



\subsubsection{Extending \PIPS~ to source-free settings}
\label{method-SFPIPS}

In this section, we explore the extension of \PIPS~ to the source-free setting \cite{liang2020we}, denoted as \PIPSSF. Crucially, in the context of \PIPSSF, the absence of $\mathcal{S}$ precludes the utilization of $\mathcal{L_{S}}$ (Equation~\ref{eqn:sup}) in training the model $\mathcal{F_{T}}$ (see Equation~\ref{eqn:overall-SF}). Additionally, as outlined in Section~\ref{method-pose2seg}, the parametric prior ($\mathcal{G}$) is typically learned using the source dataset $\mathcal{S}$. Consequently, the lack of $\mathcal{S}$ would hinder the training of $\mathcal{G}$. However, it is crucial to note that $\mathcal{G}$ does not rely on RGB images during training and is inherently domain agnostic. Even in the absence of $\mathcal{S}$, $\mathcal{G}$ could be trained using a set of paired segmentation masks ($y$) and pose keypoints ($p$) from any auxiliary dataset, similar to \cite{raychaudhuri2023prior}. Note that, assuming access to paired segmentation masks ($y$) and pose keypoints ($p$) does not violate any privacy concerns and also, significantly reduces storage requirements compared to storing the entire source dataset. 

\subsubsection{Estimating pose keypoints on target dataset}
\label{method-UDA-Pose}

As described in \cite{zhang2019unsupervised, jiang2021regressive, kim2022unified, raychaudhuri2023prior}, pose estimation models often face challenges related to domain shift. Given that we rely on pose keypoints derived from a pre-existing pose estimation model in the target domain $\mathcal{T}$ to extract anatomical information, adapting the pose model to $\mathcal{T}$ is preferable for enhancing performance. To this end, we use UDAPE \cite{kim2022unified} for \PIPS~ and POST \cite{raychaudhuri2023prior} for \PIPSSF~ to estimate pose keypoints on the target dataset $\mathcal{T}$.

\subsection{Overall Objective Function}
\label{sec-overallobj}
Our final adaptation objective for \PIPS~ is given below,
\begin{equation}
    \min_{\mathcal{F_{T}}} \;\; \eta_{1} \mathcal{L}_{S} + \eta_{2} \mathcal{L}_{p2s} + \eta_{3} \mathcal{L}_{Rpl} \ ,
    \label{eqn:overall}
\end{equation}
where $\{\eta_{i}\}_{i=1}^3$ are hyperparameters which control the contribution of individual loss terms. For our extended algorithm \PIPSSF~, $\eta_{1}$ is set to 0, as the source dataset is absent in source-free settings. Thus, our objective for \PIPSSF~ reduces to \begin{equation}
        \min_{\mathcal{F_{T}}} \;\; \eta_{2} \mathcal{L}_{p2s} + \eta_{3} \mathcal{L}_{Rpl} \ .
    \label{eqn:overall-SF}
\end{equation}

%\dripta{use something else than pi}

==> sections/4_experiments.tex <==
\section{Method}
\label{sec:method}
%
In this section, we provide a detailed description of our proposed algorithm (\PIPS) for human body part segmentation under distribution shifts. Our primary aim is to learn a human parsing model $\mathcal{F}$, which takes an RGB image $x \in$ $\mathbb{R}^{H \times W \times 3}$ as input, and predicts the segmentation mask $y = \mathcal{F}(x)$, where $y \in$ $\mathbb{R}^{H \times W \times K}$ for each of the $K$ classes. Here, $H$ and $W$ refer to the spatial dimensions of the image and the resulting segmentation output. 

We assume access to a source dataset $\mathcal{S} = \{x_{i}, y_{i}, p_{i} \}_{i=1}^{M}$, where $x_{i}$ is an RGB image, $y_{i}$ and $p_{i}$ are the corresponding segmentation masks and pose keypoints, respectively. The pose keypoints provide additional anatomical information about the human in a given image. Note that, unlike the segmentation masks, the keypoints are \textit{sparse} annotations. Additionally, we are provided with an unlabeled target dataset $\mathcal{T}$, which contains images $ \{ x_{i} \}_{i=1}^{N}$ but lacks both body part segmentation masks and pose keypoint annotations. 
%\dripta{H,W not defined}
%\dripta{usage of pose keypoints not explained}

We seek to adapt a model that has been trained on the source dataset, denoted as $\mathcal{F_{\mathcal{S}}}$, to obtain improved performance on the target dataset $\mathcal{T}$, assuming the availability of source data. This adaptation process is driven by the anatomical information provided by the pose keypoints and is designed to yield superior results compared to directly applying $\mathcal{F_{\mathcal{S}}}$ on $\mathcal{T}$. Note that pose keypoints on $\mathcal{T}$ are \textit{not} available. This requires estimation of pose keypoints on $\mathcal{T}$ using a pre-trained pose estimation model $\mathcal{P}$ (Section~\ref{method-UDA-Pose}). We denote the model under adaptation for $\mathcal{T}$ as $\mathcal{F_{\mathcal{T}}}$. 

We also extend our algorithm (\PIPS) to the source-free setting \cite{liang2020we} and denote this algorithm as \PIPSSF~(Section~\ref{method-SFPIPS}). Here, we assume that only $\mathcal{F_{S}}$ is available and do not assume the availability the source dataset $\mathcal{S}$ for our extended algorithm \PIPSSF. \\

\begin{figure*}[t]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/PIPS-method.drawio.pdf}
    \caption{ \textbf{Overview of proposed framework.} Our proposed algorithm \PIPS~uses confident pseudo-labels from $\mathcal{F_{T}}$ to refine the predictions of the same on unlabeled data $\mathcal{T}$. Further, \PIPS~leverages anatomical context of the human body through pose estimates (obtained from $\mathcal{P}$) aligned with body part segmentation masks by $\mathcal{G}$. Note that \PIPS~can be extended to source-free settings, where $\{ x_{s}, y_{s} \}$ are absent (elaborated in Section~\ref{method-SFPIPS}). Even in the absence of source-data, the anatomical context obtained from $\mathcal{G} \circ \mathcal{P}$ acts as a strong regularizer, mitigating catastrophic forgetting and compensating for domain shifts.}
    \label{fig:method}
    % \vskip -4mm
\end{figure*}

\noindent {\bf Overview:} We propose to use an anatomy guided pseudo-labelling technique to obtain improved human body part segmentation masks on $\mathcal{T}$. We note that, using the model $\mathcal{F_{\mathcal{S}}}$ directly on $\mathcal{T}$ results in notably inaccurate segmentation masks, as qualitatively illustrated in Figure~\ref{fig:teaser_qual}. Employing these inaccurate masks as pseudo-labels for adaptation would introduce error accumulation, ultimately leading to subpar performance on $\mathcal{T}$. Consequently, we introduce \PIPS, an enhanced pseudo-labeling technique that consists of two highly effective methods to circumvent this error accumulation issue: 
%\amit{You can save significant space by reducing itemsep and leftalign with itemize. Also, some of the short subsections can be combined together with paragraph headings. This is better than \vskip.}
\begin{itemize} 

    \item In order to exploit the anatomical information of the human body, we propose to fuse information from the estimated pose-keypoints on $\mathcal{T}$ (see Section~\ref{method-UDA-Pose}). This allows $\mathcal{F_{\mathcal{T}}}$ to understand the human body parts better and eliminate inconsistencies caused by self-learning from confident yet incorrect pseudo-labels (see Section ~\ref{method-pose2seg}). 

    \item Further, we propose to use the human pose context for reliable pseudo-label selection, thereby disallowing $\mathcal{F_{\mathcal{T}}}$ to overfit to incorrect but confident pseudo-labels (see Section ~\ref{method-RPL}).

\end{itemize}
An overview of our method is presented in Figure~\ref{fig:method}.
%\noindent 
%\dripta{where is the anatomical information coming from? where do you get the pose from on target?}


\begin{comment}
\subsection{Image level alignment using Style Transfer}
\label{method-style}

Style-Transfer methods have been extensively used in problems involving unsupervised domain adaption \cite{atapour2018real, rodriguez2019domain, luo2020adversarial} in order to reduce the domain gap between the source and target images. The core idea is to train a model using the content from source images while adapting to the style of target images enhances the model's ability to generalize effectively to the target distribution and has been shown to be effective in prior works like \cite{kim2020learning, yang2020fda}. 

In this work, we employ AdaIN \cite{huang2017arbitrary} for obtaining style-transfer mappings between source and target distributions and vice-versa. The style transfer network $T$ takes in style images $s$ and content images $c$ in order to learn a combination that outputs the content of the latter in the style of the former. 
Mathematically, \begin{equation}
    T(c,s) = g(AdaIN(f(c), f(s)))
\end{equation} where

Here, $g$ is a randomly initialized decoder network and $f$ is a pre-trained feature extractor such as VGG-16 \cite{simonyan2014very}. $T$ is trained using a linear combination of content loss and style loss\cite{li2017demystifying}.
 
With a pre-trained style-transfer network $T$, we project the images from $\mathcal{S}$ to the style of $\mathcal{T}$ (denoted as $x_{s \shortrightarrow t}$) and minimize the loss described by Equation~\ref{eqn:sup}, 
\begin{equation}
    \mathcal{L}_{S} = \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{s \shortrightarrow t}), y) \ .
    \label{eqn:sup}
\end{equation}
Here, $\mathcal{L}_{ce}$ denotes the per-pixel cross-entropy loss.
\end{comment}

\subsection{Pre-training source model}
We initialize the weights of $\mathcal{F}_{T}$ by the weights of a model that is trained on the labeled source domain in supervised fashion, referred to as the source model. This source model ($\mathcal{F}_{S}$) is trained by minimizing the loss described by Equation~\ref{eqn:sup}. 
\begin{equation}
    \mathcal{L}_{S} = \mathcal{L}_{ce}(\mathcal{F_{S}}(x_{s}), y) \ .
    \label{eqn:sup}
\end{equation}
Here, $\mathcal{L}_{ce}$ denotes the per-pixel cross-entropy loss.


\subsection{Self-learning from pseudo-labels}
\label{method-SL-PL}
Self-learning from pseudo-labels \cite{choi2019pseudo, wang2020unsupervised, zhang2021prototypical} offers a simple yet powerful solution in semi/self-supervised learning problems. The fundamental idea here is to utilize only highly confident pseudo-labels for learning as discussed in \cite{guillory2021predicting}. Pseudo-labels on $\mathcal{T}$, denoted by $\hat{y}_{pl}$ can be obtained by 
\begin{equation}
    \hat{y}_{pl}(\tau) = \argmax \mathbbm{1} [ \mathcal{F_{\mathcal{T}}}(x_{t}) \geq \tau ] \; \mathcal{F_{\mathcal{T}}}(x_{t}) \ ,
    \label{eqn:SL-PL}
\end{equation}  where $\tau$ is the confidence threshold and $\mathbbm{1}[.]$ is an indicator function. Note that the quality of the pseudo-labels is a function of the confidence threshold $\tau$.

These pseudo-labels are incorporated in the adaptation process by minimizing the loss $\mathcal{L}_{pl}$ defined by Equation~\ref{eqn:tgt-PL}, 
%
\begin{equation}
    \mathcal{L}_{pl}(\tau) = \mathcal{L}_{ce}(\mathcal{F_{\mathcal{T}}}(x_{t}), \hat{y}_{pl}(\tau)) \ .
    \label{eqn:tgt-PL}
\end{equation}
%    
Nevertheless, we observe that depending solely on these pseudo-labels for the adaptation process results in sub-optimal performance, as it overlooks crucial anatomical information associated with the human body. Additionally, the incorporation of highly confident yet incorrect pseudo-labels can adversely affect the overall adaptation process.

\subsection{Anatomy guided self-training}
\label{method-pose2seg}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/PIPS-learning_G.drawio.pdf}
    \caption{\textbf{Learning algorithm for $\mathcal{G}$}. The model $\mathcal{G}$ is designed to predict segmentation maps $\hat{s} \in \mathbb{R}^{H \times W \times K}$ given pose keypoints $p \in \mathbb{R}^{P \times 2}$. $\mathcal{G}$ is trained using the cross-entropy loss with ground-truth segmentation maps $s \in \mathbb{R}^{H \times W \times K}$.}
    \label{fig:pose2seg}
    \vskip -4mm
\end{wrapfigure}

To utilize anatomical information from pose keypoints for adapting our model $\mathcal{F_{T}}$ to the target dataset $\mathcal{T}$, we propose learning a mapping $\mathcal{G}$ that transforms sparse pose keypoints to dense body part segmentation masks. Here, $\mathcal{G} : \mathbb{R}^{P \times 2} \shortrightarrow \mathbb{R}^{H \times W \times K}$, with $P$ representing the number of pose keypoints and $K$ denoting the number of classes in the segmentation maps (e.g., head, left/right leg, etc.).

The mapping $\mathcal{G}$ is learnt in a supervised fashion using our source dataset $\mathcal{S} = \{x_{i}, y_{i}, p_{i} \}_{i=1}^{M}$ by minimizing the loss in Equation~\ref{eqn:L-G}, 
\begin{equation}
        \mathcal{L_{G}} = \mathcal{L}_{ce}(\mathcal{G}(p_{j}), y_{j})  \ .
    \label{eqn:L-G}
\end{equation}
It is important to note that the learning of $\mathcal{G}$ does not use any RGB images, thus making it domain agnostic and hence, seamlessly applicable across different domains. Figure~\ref{fig:pose2seg} provides an overview for the learning algorithm of $\mathcal{G}$.

%\amit{Is this the best place to introduce the SF approach? Wouldn't it be better to do the next section first, and then have a new section on the source-free approach? I think that will help with the flow of the paper in the reviewers' minds.}

\begin{comment}
    \begin{figure}[t]
        \centering
        \includegraphics[width=0.8\columnwidth]{images/PIPS-learning_G.drawio.pdf}
        \caption{ \textbf{Learning algorithm for $\mathcal{G}$}. The model $\mathcal{G}$ is designed by predict segmentation maps $\hat{s} \in \mathbb{R}^{H \times W \times K}$ given pose keypoints $p \in \mathbb{R}^{P \times 2}$. $\mathcal{G}$ is trained using the cross-entropy loss with ground-truth segmentation maps $s \in \mathbb{R}^{H \times W \times K}$.}
        \label{fig:pose2seg}
        \vskip -4mm
    \end{figure}
\end{comment}

Using the learned mapping $\mathcal{G}$ we can extract anatomically plausible pseudo-labels on the target dataset $\mathcal{T}$, however, this requires access to pose keypoint annotations on $\mathcal{T}$. Since we do not have access to any annotations on $\mathcal{T}$, we propose to estimate the same using a pre-trained pose estimation model which has been adapted on $\mathcal{T}$ (see Section ~\ref{method-UDA-Pose} for details).

%The learned mapping $\mathcal{G}$ is now used to extract pseudo-labels for target images $x_{t}$ via a pretrained human pose estimation model $\mathcal{P}$ (see Section ~\ref{method-UDA-Pose}). 

Mathematically, pseudo-labels $\hat{y}_{p2s}$ are obtained by \begin{equation}
    \hat{y}_{p2s} = \mathcal{G} \circ \mathcal{P} (x_{t}) \ ,
    \label{eqn:p2s}
\end{equation} and are used in the adaptation process by minimizing the loss function described in Equation~\ref{eqn:L-P2S}, 

%\dripta{describe pose more: why do you use it? how do you obtain it (in brief) Maybe add a sentence: Let us assume that we have access to a pose estimation model.... We describe the details of how to obtain this model in Sec x.}

\begin{equation}
    \mathcal{L}_{p2s} = \mathcal{L}_{ce}(\mathcal{F_{\mathcal{T}}}(x_{t}), \hat{y}_{p2s})
    \label{eqn:L-P2S} \ .
\end{equation} 

Incorporating the loss function from Equation~\ref{eqn:L-P2S} along with losses in Equations~\ref{eqn:sup} and~\ref{eqn:tgt-PL} contributes significantly to the improvement of $\mathcal{F_{T}}$ over the base source model. However, using pose information solely as a regularizer is insufficient, as $\mathcal{F_{T}}$ may still overfit to highly confident but incorrect pseudo-labels, leading to sub-optimal performance. Therefore, we recommend utilizing the anatomical context from Equation~\ref{eqn:p2s} to enhance the refinement of pseudo-labels $\hat{y}_{pl}$, thus driving additional performance enhancements.

\subsection{Pose-guided reliable pseudo-label selection}
\label{method-RPL}
In order to make our method more robust to incorrect pseudo-labels, we wish to employ an approach that helps $\mathcal{F_{T}}$ avoid learning from highly-confident incorrect pseudo-labels. We argue that the quality of pseudo-labels obtained using Equation~\ref{eqn:SL-PL} on a given batch of images from $\mathcal{T}$ is not homogeneous. In other words, for a batch of target images, a single threshold parameter $\tau$ may not be an optimal choice. Taking inspiration from Karim {\it et al.} \cite{karim2023c}, we argue that any batch of target images consists of reliable and unreliable samples. In other words, predictions for some samples are relatively more accurate as compared against other samples from the same batch. Thus, we propose to split a given batch of target images (denoted by $x_{t}^{\mathbf{B}}$, containing $\mathbf{B}$ images) into reliable and unreliable splits containing $\mathbf{B}^{r}$ and $\mathbf{B}^{u}$ images respectively.

These splits are obtained by comparing the mIoU \cite{rezatofighi2019generalized} of the predictions $\mathcal{F_{T}}(x_{t})$ with $\hat{y}_{p2s}$. Essentially, for the $j^{th}$ image in a batch of target images, we obtain a score $h^{j}$ defined by Equation~\ref{miou-com},
\begin{equation}
    \label{miou-com}
    h^{j} = mIoU(\mathcal{\argmax(F_{T}}(x^{j}_{t})), \hat{y}^{j}_{p2s}) \ .
\end{equation}
%
This score $h^{j}$ is then used to decompose a batch of $\mathbf{B}$ images into reliable and unreliable splits as follows, 
\begin{equation}
    x_{t}^{\mathbf{B}}= 
    \begin{dcases}
         x_{t}^{r}, & \text{$h_{j}$} \geq \gamma\\
         x_{t}^{u}, & \text{otherwise}
    \end{dcases} \ ,
    \label{eqn:split}
\end{equation}
where $\gamma$ is the threshold defining the boundary between reliable and unreliable samples. 

\begin{comment}
    = $\frac{\sum_{j=1}^{\mathbf{B}}h^{j}}{|\mathbf{B}|}$
\end{comment}

This is followed by extracting the confident pseudo-labels using Equation~\ref{eqn:SL-PL} with confidence thresholds $\alpha$ and $\beta$ with $\beta \geq \alpha$, for reliable and unreliable splits respectively. These pseudo-labels are now incorporated into the framework using the loss function defined below,
\begin{equation}
    \begin{split}
        \mathcal{L}_{Rpl} & = \lambda \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{t}^{r}), \hat{y}_{pl}(\alpha)) + (1 - \lambda) \mathcal{L}_{ce}(\mathcal{F_{T}}(x_{t}^{u}),  \hat{y}_{pl}(\beta)) \ .
    \label{eqn:loss-RPL}
    \end{split}
\end{equation}
%
Here, $\lambda$ is set to $\frac{|\mathbf{B^{r}}|}{|\mathbf{B}|}$. We experimentally demonstrate that this strategy of pseudo-label selection during adaptation contributes significantly to the overall performance gains of \PIPS~.
\begin{comment}
\begin{figure}[!htb]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/Teaser final sf_posture.png}
    \caption{{\bf Overview of \PIPSSF~.} We extend our problem definition to look into source-free UDA for human body part segmentation, thereby addressing privacy and storage bottlenecks associated with using source data for adaptation as in \PIPS~.}
    \label{fig:teaser_sfposture}
\end{figure}
\end{comment}
    
\subsection{Estimating pose keypoints on target dataset}
\label{method-UDA-Pose}

As described in \cite{zhang2019unsupervised, jiang2021regressive, kim2022unified, raychaudhuri2023prior}, pose estimation models often face challenges related to domain shift. Given that we rely on pose keypoints derived from a pre-existing pose estimation model in the target domain $\mathcal{T}$ to extract anatomical information, adapting the pose model to $\mathcal{T}$ is preferable for enhancing performance. To this end, we use UDAPE \cite{kim2022unified} for \PIPS~to estimate pose keypoints on the target dataset $\mathcal{T}$. However, it is important to note that, \emph{while adaptation of the pose estimation model ($\mathcal{P}$) to the particular target domain ($\mathcal{T}$) gives superior human body part segmentation masks, this step is not mandatory to the success of \PIPS. In fact, in Section~\ref{sec:abl} (Table~\ref{tab:imp-poseadapt}) we show that an unadapted pose estimation model can also deliver significant performance gains.} 

\subsection{Overall Objective Function}
\label{sec-overallobj}
Our final adaptation objective for \PIPS~is given below,
\begin{equation}
    \min_{\mathcal{F_{T}}} \;\; \eta_{1} \mathcal{L}_{S} + \eta_{2} \mathcal{L}_{p2s} + \eta_{3} \mathcal{L}_{Rpl} \ ,
    \label{eqn:overall}
\end{equation}
where $\{\eta_{i}\}_{i=1}^3$ are hyperparameters which control the contribution of individual loss terms. 

\subsection{Extending \PIPS~to source-free settings}
\label{method-SFPIPS}

In this section, we explore the extension of \PIPS~to the source-free setting \cite{liang2020we}, denoted as \PIPSSF. Crucially, in the context of \PIPSSF, the absence of $\mathcal{S}$ precludes the utilization of $\mathcal{L_{S}}$ (Equation~\ref{eqn:sup}) in training the model $\mathcal{F_{T}}$ (see Equation~\ref{eqn:overall-SF}). Additionally, as outlined in Section~\ref{method-pose2seg}, the parametric prior ($\mathcal{G}$) is typically learned using the source dataset $\mathcal{S}$. Consequently, the lack of $\mathcal{S}$ would hinder the training of $\mathcal{G}$. However, it is crucial to note that $\mathcal{G}$ does not rely on RGB images during training and is inherently domain agnostic. Even in the absence of $\mathcal{S}$, $\mathcal{G}$ could be trained using a set of paired segmentation masks ($y$) and pose keypoints ($p$) from any auxiliary dataset, similar to \cite{raychaudhuri2023prior}. Note that, assuming access to paired segmentation masks ($y$) and pose keypoints ($p$) does not violate any privacy concerns and also, significantly reduces storage requirements compared to storing the entire source dataset. 

Note that, UDAPE \cite{kim2022unified} is not applicable for \PIPSSF~for pose estimation on the unlabeled target dataset ($\mathcal{T}$) because UDAPE inherently relies on using source data. Consequently, we employ POST \cite{raychaudhuri2023prior}, a recent source-free domain adaptive human pose estimation algorithm, to predict pose keypoints on $\mathcal{T}$.

For \PIPSSF, $\eta_{1}$ in Equation~\ref{eqn:overall} is set to 0, as the source dataset is absent in source-free settings. Thus, our objective for \PIPSSF~reduces to \begin{equation}
        \min_{\mathcal{F_{T}}} \;\; \eta_{2} \mathcal{L}_{p2s} + \eta_{3} \mathcal{L}_{Rpl} \ .
    \label{eqn:overall-SF}
\end{equation}


